TPCpp-10M: Simulated proton-proton collisions in a Time Projection Chamber for AI Foundation Models

Scientific foundation models hold great promise for advancing nuclear and particle physics by improving analysis precision and accelerating discovery. Yet, progress in this field is often limited by the lack of openly available large scale datasets, as well as standardized evaluation tasks and metrics. Furthermore, the specialized knowledge and software typically required to process particle physics data pose significant barriers to interdisciplinary collaboration with the broader machine learning community. This work introduces a large, openly accessible dataset of 10 million simulated proton-proton collisions, designed to support self-supervised training of foundation models. To facilitate ease of use, the dataset is provided in a common NumPy format. In addition, it includes 70,000 labeled examples spanning three well defined downstream tasks: track finding, particle identification, and noise tagging, to enable systematic evaluation of the foundation model's adaptability. The simulated data are generated using the Pythia Monte Carlo event generator at a center of mass energy of sqrt(s) = 200 GeV and processed with Geant4 to include realistic detector conditions and signal emulation in the sPHENIX Time Projection Chamber at the Relativistic Heavy Ion Collider, located at Brookhaven National Laboratory. This dataset resource establishes a common ground for interdisciplinary research, enabling machine learning scientists and physicists alike to explore scaling behaviors, assess transferability, and accelerate progress toward foundation models in nuclear and high energy physics. The complete simulation and reconstruction chain is reproducible with the sPHENIX software stack. All data and code locations are provided under Data Accessibility.

==> macro.tex <==
% dataset name
\newcommand{\trackml}{\texttt{TrackML}\xspace}
\newcommand{\sphenix}{\texttt{sPHENIX}\xspace}
\newcommand{\tpcpp}{\texttt{TPCpp-10M}\xspace}
\newcommand{\ppcol}{$p{+}p$\xspace}

% model names:
\newcommand{\maskformer}{\texttt{MaskFormer}\xspace}
\newcommand{\masktwoformer}{\texttt{Mask2Former}\xspace}
\newcommand{\eggnet}{\texttt{EggNet}\xspace}
\newcommand{\exatrkx}{\texttt{Exa.TrkX}\xspace}
\newcommand{\fm}{\texttt{FM4NPP}\xspace}
\newcommand{\fmmvi}{\texttt{FM4NPP(m6)}\xspace}
\newcommand{\fmhead}{\texttt{AdapterOnly}\xspace}
\newcommand{\GATConv}{\texttt{GATConv}\xspace}
\newcommand{\GCNConv}{\texttt{GCNConv}\xspace}
\newcommand{\GraphConv}{\texttt{GraphConv}\xspace}
\newcommand{\SAGEConv}{\texttt{SAGEConv}\xspace}
\newcommand{\oneformer}{\texttt{OneFormer3D}\xspace}
\newcommand{\gravnet}{\texttt{GravNet}\xspace}

% write physcal quantity with unit in a principled way:
\newcommand{\gev}[1]{\SI{#1}{\giga\electronvolt}}
\newcommand{\mev}[1]{\SI{#1}{\mega\electronvolt}}
\newcommand{\pt}{\ensuremath{p_{\mathrm{T}}\xspace}}
% physics related terms
\newcommand{\geant}{\textsc{Geant4}\xspace}
\newcommand{\pythia}{\textsc{Pythia}\xspace}



% delimiters:
\newcommand{\paren}[1]{\left(#1\right)}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\bracket}[1]{\left[#1\right]}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}

% alerts
\newcommand{\addcitation}{\textcolor{red}{[ADD CITATION]}\xspace}
\newcommand{\pleasecheck}{\textcolor{red}{[PLEASE CHECK]}\xspace}
\newcommand{\adddetails}[1]{\textcolor{green}{ADD DETAILS on {#1}}\xspace}

% color for classes
\definecolor{pion}{HTML}{66C2A5}
\definecolor{kaon}{HTML}{FC8D62}
\definecolor{proton}{HTML}{8DA0CB}
\definecolor{electron}{HTML}{E78AC3}
\definecolor{others}{HTML}{A6D854}
\definecolor{signal}{HTML}{00BFFF}
\definecolor{noise}{HTML}{FF7F50}

% author comments
\definecolor{BrickRed}{rgb}{0.8, 0.25, 0.33}
\definecolor{DarkGreen}{rgb}{0.0, 0.4, 0.0}
\definecolor{RoyalBlue}{rgb}{0.25, 0.41, 0.88}
\definecolor{Orchid}{rgb}{0.85, 0.44, 0.84}
\definecolor{ProcessCyan}{rgb}{0.0, 0.68, 0.93}
\definecolor{DarkOrange}{rgb}{1.0, 0.55, 0.0}
\definecolor{Brown}{rgb}{0.65, 0.16, 0.16}
\definecolor{OliveGreen}{rgb}{0.33, 0.42, 0.18}
\definecolor{BlueViolet}{rgb}{0.54, 0.17, 0.89}
\definecolor{MidnightBlue}{rgb}{0.1, 0.1, 0.44}
\definecolor{Goldenrod}{rgb}{0.85, 0.65, 0.13}
\newcommand{\ray}[1]{\textcolor{BrickRed}{[Ray: #1]}}
\newcommand{\david}[1]{\textcolor{DarkGreen}{[David: #1]}}
\newcommand{\jin}[1]{\textcolor{RoyalBlue}{[Jin: #1]}}
\newcommand{\shuhang}[1]{\textcolor{Orchid}{[Shuhang: #1]}}
\newcommand{\shinjae}[1]{\textcolor{ProcessCyan}{[Shinjae: #1]}}
\newcommand{\yi}[1]{\textcolor{DarkOrange}{[Yi: #1]}}
\newcommand{\joe}[1]{\textcolor{Brown}{[Joe: #1]}}
\newcommand{\haiwang}[1]{\textcolor{OliveGreen}{[Haiwang: #1]}}
\newcommand{\yeonju}[1]{\textcolor{BlueViolet}{[Yeonju: #1]}}
\newcommand{\xihaier}[1]{\textcolor{MidnightBlue}{[Xihaier: #1]}}
\newcommand{\yuewei}[1]{\textcolor{Goldenrod}{[Yuewei: #1]}}
